Topo4D: Topology-Preserving Gaussian Splatting for High-Fidelity 4D Head Capture

4D head capture aims to generate dynamic topological meshes and corresponding texture maps from videos, which is widely utilized in movies and games for its ability to simulate facial muscle movements and recover dynamic textures in pore-squeezing. The industry often adopts the method involving multi-view stereo and non-rigid alignment. However, this approach is prone to errors and heavily reliant on time-consuming manual processing by artists. To simplify this process, we propose Topo4D, a novel framework for automatic geometry and texture generation, which optimizes densely aligned 4D heads and 8K texture maps directly from calibrated multi-view time-series images. Specifically, we first represent the time-series faces as a set of dynamic 3D Gaussians with fixed topology in which the Gaussian centers are bound to the mesh vertices. Afterward, we perform alternative geometry and texture optimization frame-by-frame for high-quality geometry and texture learning while maintaining temporal topology stability. Finally, we can extract dynamic facial meshes in regular wiring arrangement and high-fidelity textures with pore-level details from the learned Gaussians. Extensive experiments show that our method achieves superior results than the current SOTA face reconstruction methods both in the quality of meshes and textures. Project page: https://xuanchenli.github.io/Topo4D/.

==> Figures/Face_Reconstruction/quality_cmp.tex <==
\begin{figure*}[!hbtp]
    \centering
    \begin{minipage}{1\linewidth}
        \centering
        \begin{minipage}{1\linewidth}
            \centering
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/SQ_01_600.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/DECA.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/3DDFA.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/HRN.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/MVFR.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/DFNRMVS.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/ICP.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/ours.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/SQ_01_600/GT.png}
            \end{minipage}
        \end{minipage}

        \begin{minipage}{1\linewidth}
            \centering
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/WJY_01_80.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/DECA.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/3DDFA.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/HRN.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/MVFR.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/DFNRMVS.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/ICP.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/ours.png}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/WJY_01_80/GT.png}
            \end{minipage}

        \end{minipage}

        \begin{minipage}{1\linewidth}
            \centering
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/ZQ_mbs_120.png}
                \captionsetup{font=tiny}
                \caption*{Front View}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/DECA.png}
               \captionsetup{font=tiny}
                \caption*{DECA}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/3DDFA.png}
                \captionsetup{font=tiny}
                \caption*{3DDFA}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/HRN.png}
                \captionsetup{font=tiny}
                \caption*{HRN}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/MVFR.png}
                \captionsetup{font=tiny}
                \caption*{MVFR}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/DFNRMVS.png}
                \captionsetup{font=tiny}
                \caption*{DFNRMVS}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/ICP.png}
                \captionsetup{font=tiny}
                \caption*{MVS+ICP}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/ours.png}
                \captionsetup{font=tiny}
                \caption*{ours}
            \end{minipage}
            \begin{minipage}{0.1\linewidth}
                \includegraphics[width=1\linewidth]{Figures/Face Reconstruction/quality_cmp/ZQ_mbs_120/GT.png}
                \captionsetup{font=tiny}
                \caption*{GT}
            \end{minipage}
        \end{minipage}
    \end{minipage} 
    \captionof{figure}{Qualitative evaluation.}
    \label{fig:quality_cmp}
\end{figure*}


==> Figures/rebuttal/multiface.tex <==
\begin{figure}[t]
	\centering
        % \vspace{-1em}
	\includegraphics[width=\linewidth]{Figures/rebuttal/multiface.png}
 \vspace{-2.25em}
	\caption{Comparisons on Multiface Dataset. Challenging areas are highlighted in red boxes. Please \textbf{zoom-in}.}
        \vspace{-1.25em}
	\label{img:multiface_supp}
\end{figure}

==> Tables/Attributes.tex <==
\begin{table}[tb]
\centering
\caption{The initialization settings and learning strategies for each Gaussian attribute.}
\label{tbl:attributes}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Symbol} & \textbf{Initialization} & \textbf{First Frame} & \textbf{Subsequent Frames} \\ \hline
$\mu$              & Vertex Coordinate     & Fixed                             & Learnable                        \\ \hline
$q$                & Vertex Normal          & Learnable                         & Learnable                        \\ \hline
$s$                & Half of Min Neighbour Distance  & Learnable                         & Fixed                            \\ \hline
$\sigma$           & 1                       & Fixed                             & Fixed                            \\ \hline
$c$                & Texture Color           & Fixed                             & Learnable                        \\ \hline
\end{tabular}%
}
\end{table}

==> Tables/time.tex <==
\begin{table}[htbp]
\caption{Time required per frame.}
\tiny
\centering
\resizebox{0.38\textwidth}{!}{%
\begin{tabular}{c|c|c}
\toprule
Method                           & Mesh   & Texture \\ 
\midrule
traditional pipeline             & $>$30min & $>$3min   \\
Fyffe et al. (EUROGRAPHICS 2017) & $>$40min & -       \\
Ours                             & 30s    & 30s     \\ \bottomrule
\end{tabular}%
}
\label{tbl:time}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \small
% \caption{Time required per frame under different setting.}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|c|c|c|c}
% \toprule
% Density  & w/o Densification & N = 10 & N = 20 & N = 30 \\ \hline
% Time(s) & 22.58                  & 24.91       & 29.08       & 45.94       \\ \bottomrule
% \end{tabular}%
% % }
% \label{tbl:tex_time}
% \end{table}
% \begin{table}[ht]
%   \centering
%   \caption{Time required per frame under different setting.}
%   \small % 设置表格内文字的大小为small
%   \begin{tabularx}{\textwidth}{X|c|c|c|c} % 创建一个占据整个文本宽度的表格
%     \toprule
% Density  & w/o Densification & N = 10 & N = 20 & N = 30 \\ \hline
% Time(s) & 22.58                  & 24.91       & 29.08       & 45.94       \\ \bottomrule
%   \end{tabularx}
%   \label{tbl:tex_time}
% \end{table}

==> sections/method.tex <==
\section{Methods}
\textbf{Overview.}
Our method aims to generate dynamic head meshes and temporal stable textures from calibrated multi-view videos. Specifically, given sets of multi-view image sequences $\{ \mathcal{I}^j_i \in \mathbb{R}^{h \times w \times 3} | 1 \leq i \leq F\}_{j=1}^K$ with $F$ frames from $K$ views and known camera calibrations, our method extracts head meshes $\{S_i:=(V^i, T)|V^i\in\mathbb{R}^{n_v\times3}, T\in\mathbb{R}^{n_f\times3} \}_{i=1}^F$ with predefined fixed topology $T$ that has $n_v$ vertices and $n_f$ faces together with 8K texture maps $\{M_i\in\mathbb{R}^{8196\times8196\times3} \}_{i=1}^F$.

As is illustrated in figure, our method first binds dynamic gaussians to mesh vertices by initializing a \textit{Gaussian Mesh} based on the priors from the first frame (Sec. \ref{sec:Gaussian Mesh})\todo{Sec 3.1} Then, in each subsequent frame, we perform geometry optimization (Sec. \ref{sec:Geo Opt}) and texture optimization (Sec. \ref{sec:Tex Opt}) alternately. During geometry optimization, our method combines physical prior losses with topological priors to extract geometries with fine topology. And so as to directly generate texture map with pore-level details from \textit{Gaussian Mesh}, we conduct UV space gaussian densification and texture inverse mapping that map colors from world space to UV space.
% Overview：我们的方法基于4DGS优化，输入是一组多视角视频及其相机参数，同时还有通过MVS+Registration方法生成的第一帧人脸几何和贴图。我们用第一帧的贴图和几何初始化高斯点集来构建Gaussian Mesh，为后续的优化过程提供了充分的拓扑、形状和颜色先验。通过物理和拓扑约束，我们优化并跟踪每个高斯点在每一帧的三维位置，从而提取出动态几何。在每一帧我们进行几何和纹理的交替优化，通过UV空间顶点稠密化，我们可以学习精确的顶点颜色并生成原生8K纹理。接下来我们首先介绍GS的前置知识，再给出第一帧初始化并优化Gaussian Mesh的方法。之后我们将详细介绍后续每一帧对几何和纹理的交替优化方法。
\subsection{Preliminary}
3D Gaussian Splatting (3DGS)~\cite{3DGS} is proposed as a competitive solution to represent and render static scenes. Different from other implicit representation methods, 3DGS explicitly maintains a set of Gaussians to model a scene. By virtue of the explicit intrinsics of Gaussians and the absence of dense MLP execution when sampling from scene representation, 3DGS can render scenes effciently while maintaining high fidelity. Each ellipsoidal Gaussian is described by a covariance matrix $\Sigma$ and its mean position $\mu$:\begin{equation}G(x)=e^{-\frac{1}{2} (x)^T\Sigma ^{-1}(x)}\end{equation} In order to ensure positive definiteness of the covariance matrix to guarantee its physical meaning during the gradient descent optimization process, $\Sigma$ is further decomposed into rotation matrix $R$ and scaling matrix $S$:\begin{equation}\Sigma=RSS^TR^T\end{equation}, where the rotation matrix is parameterized using a quaternion $q$ for the sake of optimization convenience. In addition to these attributes, each Gaussian also features a learnable color component $c$ and an opacity component $\sigma$ used for rendering.

For rendering, all 3D Gaussians are projected to 2D image plane\cite{zwicker2001ewa}:\begin{equation}\Sigma^\prime=JW\Sigma W^TJ^T\end{equation}, where $W$ is the viewing transformation matrix and $J$ is the Jacobian of the affine approximation of the projective
transformation. Finally, the color $C$ of a pixel is acquired by sampling and blending all Gaussians that overlapping the pixel 
in depth order: \begin{equation}C=\sum_{i=1}c_i\alpha_i\prod_{j=1}^{i-1}(1-\alpha_i)\end{equation}, where the blending weight $\alpha_i$
is given by evaluating a 2D Gaussian with its covariance multiplied with its opacity.

However, 3DGS is designed for rendering, not for 3D reconstruction. There is no topological relationship between Gaussians, and unconstrained optimization of their attributes can only produce meaningless geometry, making it impossible to directly extract topologically good meshes.
% Preliminary：GS能从带有位姿的多视角图进行快速高分辨率渲染，通过在第一帧优化高斯的属性，并在后续帧约束这些属性，可以通过多视角图像的变化驱动这些高斯点；{Gaussian Splatting的符号、表示、投影、渲染方程；}
% GS的优势
% GS通过分布在空间中的Gaussian混合颜色实现渲染，然而高斯点之间没有拓扑关系，不加约束地优化三维坐标会导致没有意义的几何形状，无法直接提取拓扑好的mesh和texture；

\subsection{Gaussian Mesh: Topology Integrated Gaussians Initialization}
\label{sec:Gaussian Mesh}
\todo{simplify}3DGS can efficiently render scenes with high fidelity, but does not have meaningful geometry. Meanwhile, explicit mesh is easy to control, but difficult to be reconstructed effectively by multi-view videos. To solve the problem mentioned above and have the best of both worlds, we propose \textit{Gaussian Mesh} by integrating topological priors to the initialization and subsequent frame by frame optimization process of vanilla Gaussians.

\todo{sup.mat. Attributes table}

% \input{Tables/Attributes} 
\todo{rename}\noindent{\bf Gaussian Mesh Initialization.}
Different from 3DGS using SFM to generate sparse point clouds for Gaussian initialization, our method begins from a head mesh and texture of the first frame, which is acquired by a off the shelf automatic MVS and registration method. The mesh and texture of the first frame provide reliable geometry and color information, together with the predefined topology. Our goal is to introduce these priors to Gaussians and directly extract geometry from the mean positions $\mu$ of Gaussians, so we initialize Gaussians $G_1=\{G_{1,i}\}_{i=1}^{n_v}$ with the same number of vertices in the mesh, and set the mean position of Gaussians to the vertex 3D world space coordinates in topological order. At the same time, in order to avoid color blending between multiple Gaussians as much as possible, and to form a one-to-one correspondence between the facial region and the Gaussians, we initialize the scales $s$ as the minimum distance between each vertex and its one-ring neighbors ($ORN$), and set opacity $\sigma$ to 1. All in all, the proposed Gaussian Mesh is composed of a set of constrained optimized Gaussians as shown in Tab. \ref{tbl:attributes}.
% Topology Integrated Gaussians initialization：与普通的3DGS使用SFM产生的稀疏点云初始化高斯点集不同，我们首先用传统MVS+Fitting的方式重建出第一帧的mesh和texture作为拓扑和颜色先验，再将Gaussian分布绑定到第一帧的人脸网格。由于希望能够从高斯点的位置直接提取出几何，我们创建与网格顶点数目相同的高斯点，将高斯的mean position按照拓扑顺序设置为网格顶点坐标；同时为了尽可能避免多个高斯间的颜色混合，使面部区域与高斯点集尽可能构成一一对应，我们将scale初始化为每个顶点与其one-ring neighbour距离的最小值，并设置每个高斯的opacity为1；

% 总之，Gaussian Mesh由一组限制优化的Dynamic Gaussian组成：
% （1）mean position，代表了每一帧对应的网格顶点，网格顶点和高斯保持一致一一对应（第一帧保持不变、后续帧可学习）
% （2）rgb空间颜色（第一帧保持不变、后续帧可学习）
% （3）scale（第一帧可学习、后续帧保持不变）
% （4）opacity（设置为1，保持不变）
% （5）rotation（可学习）

% \todo{}Notably, GaussianAvatar~\cite{GaussianAvatar} also utilizes face priors by rigging Gaussians to explicit head mesh, and drive it by FLAME\cite{FLAME} parameters. However \cite{GaussianAvatar} rigs multiple Gaussians to mesh faces while we bind a single Gaussian to each vertex and build a a one-to-one mapping between Gaussians and vertices according to the topology. 
\todo{guodu:chu shi hua hou you hua yuan yin}
\todo{rename}\textbf{First Frame Optimization.} For we have known the reliable geometry and color priors of the first frame head, we only need to optimize Gaussians' scale and rotation. The first frame optimization stage uses the same image loss as 3DGS:\begin{equation}\label{loss:image}\mathit{L}_{image} = (1-\lambda ) \mathit{L}_{1} + \lambda\mathit{L}_{D-SSIM}\end{equation}, where $\lambda$ is always set to 0.2.
Since a Gaussian is like an ellipsoid but a point without volume, and its mean position does not represent the true position of the surface it renders. If we want to extract geometry from Gaussians directly, we need to hypothesize that the Gaussians are like flat ellipses and aligned with the underlying head surface closely. This actually requires constraining one direction of Gaussian's scale close to 0:\begin{equation}\mathit{L}_{scale} = \Vert s \Vert_{-\infty}\end{equation}.
Overall, the final loss for Gaussian Mesh initialization can be formulated as:\begin{equation}\mathit{L}_{init} = \mathit{L}_{image} + \lambda_{scale} \mathit{L}_{scale}\end{equation}
% Next, we will articulate how to regularize the motion of dynamic Gaussians and reconstruct head Gaussian Mesh in a temporally persistent manner.
% 初始帧优化目标：由于已知第一帧的可靠几何和颜色先验，因此我们在第一帧只优化高斯的scale、rotation。初始帧优化阶段使用和3DGS相同的image损失（L1loss + ssim）:{公式和说明}
%scale损失：{公式和说明}
%接下来我们具体介绍后续帧的几何优化。
\subsection{Geometry Optimization}
\label{sec:Geo Opt}
After the first frame optimization stage, we have built a Gaussian Mesh formed by the Gaussian set $G_1$. Next, our method will optimize Gaussian attributes under the regulation of physical and topology priors. The Gaussian set $G_i$ at frame $i$ is acquired by optimizing $G_{i-1}$ at the previous frame. 

The learning strategies for each attribute are illustrated in Tab. \ref{tbl:attributes}. By initializing the RGB/position of Gaussians with a reliable prior in the first frame, each 3D Gaussian can represent the physical components of the corresponding facial position. By freezing the scale in subsequent frames while releasing rotation and position, the motion of the corresponding physical components of the face can be modeled. It is worth noting that the same facial region will produce different colors when doing different expressions, e.g. ambient occlusion around wrinkles. Therefore, by allow Gaussian's color change during optimization, we can to some extent model shadows caused by self occlusion. The facial color prior in the first frame cannot reflect this phenomenon, but it is crucial for recognizing facial geometry.

\todo{guodu: why these three}Overall, the optimization objective of geometry is constructed by three parts: \begin{equation}
    \mathit{L}_{geo} = \mathit{L}_{image} + \mathit{L}_{phy} + \mathit{L}_{topo}
\end{equation}
%通过在第一帧用可靠先验初始化高斯的rgb/position，同时设置opacity为1，可以使得每个3D高斯表示人脸相应位置的物理成分；通过在后续帧限制高斯scale，同时放开rotation和position、可以建模人脸相应物理成分的运动。
% 值得注意的是，相同的面部区域会随着表情的不同产生不同的阴影颜色，因此我们放开rgb的学习，有助于建模由于人脸动态运动导致的阴影和褶皱。第一帧的面部颜色先验无法给予这部分信息，但是对识别人脸几何十分重要。

% 几何优化：
% 几何的优化目标由3部分组成：Loss=image loss + phy loss + topo loss

\textbf{Physical Prior Loss.}
The correspondence between Gaussians and facial regions achieved by solely freezing some attributes of Gaussians is weak. For example, for regions such as forehead and cheek, where the color is similar and the geometry is relatively flat, a Gaussian can freely represent similar physical areas, leading to incorrect tracking relationships. This means that in addition to indirectly optimizing Gaussian positions through differentiable rendering, physical priors are needed to regularize the motion of Gaussians directly. Following the practice of \cite{DynamicGaussian} but with some modifications, our physical prior loss consists of three parts:\begin{equation}
    \mathit{L}_{phy} = \lambda_{rigid}\mathit{L}_{rigid} + \lambda_{rot}\mathit{L}_{rot} + \lambda_{iso}\mathit{L}_{iso}
\end{equation}, where $\mathit{L}_{rigid}$ and $\mathit{L}_{rot}$ are used to regularize short-term local-rigidity and rotation
similarity of Gaussians, respectively, and $\mathit{L}_{iso}$ is a long-term local-isometry loss. We refer readers to \cite{DynamicGaussian} for more details about the original design of these loss terms.

% 只通过冻结高斯的部分属性来实现高斯和人脸对应位置的绑定是不可靠的，例如对于额头、脸颊等区域，颜色相同且几何较为平整，一个高斯可以自由地表征相似的物理区域，导致错误的跟踪关系。
The physical loss between Gaussians should under the priors of topology for we don't want a Gaussian to affect all nearby Gaussians blindly, e.g. a Gaussian on the upper lip and a Gaussian on the lower lip but closest to it. Therefore, unlike \cite{DynamicGaussian}, we only impose such loss between one-ring neighbours:\begin{equation}
    \mathit{L}_{rigid}(i, j)=w_{i, j}\Vert(\mu_{j,t-1}-\mu_{i,t-1})-R_{i,t-1}R_{i,t}^{-1}(\mu_{j,t}-\mu_{i,t})\Vert_2
\end{equation}
\begin{equation}
    \mathit{L}_{rigid}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} \mathit{L}_{rigid}(i,j)
\end{equation}, where $n_e$ is the number of edges and $ORN_i$ means the one-ring neighbours of $G_i$. The loss weighing factor takes into account the edge length of the Gaussian Mesh at the first frame:\begin{equation}
    w_{i, j}=exp(-\lambda_w\Vert\mu_{j, 0}-\mu_{i,0}\Vert_2^2)
\end{equation}

% 刚体距离损失：{公式和说明}
We also regularize Gaussian's rotation in a similar manner:\begin{equation}
     \mathit{L}_{rot}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} w_{i,j}\Vert\hat q_{j, t}\hat q_{j, t-1}^{-1}-\hat q_{i, t}\hat q_{i, t-1}^{-1}\Vert_2
\end{equation}, where $\hat q$ is the normalized quaternion.

% 刚体旋转损失：{公式和说明}
In addition to the loss terms mentioned above that are only calculated between adjacent frames, we find that long-term physical loss is important for maintaining long-distance topological consistency after doing expressions, for it strongly introduces the topology priors about the edge length:\begin{equation}
    \mathit{L}_{iso}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} w_{i,j}|\Vert\mu_{j,0}-\mu_{i,0}\Vert_2-\Vert\mu_{j,t}-\mu_{i,t}\Vert_2|
\end{equation}

% 刚体长距离损失：{公式和说明}
\textbf{Topology Prior Loss.}
By means of the physical constraints mentioned above, it is already able to achieve long-term tracking of the corresponding face regions. But if vertices are strictly constrained by physical constraints, it can lead to clustering of vertices in some cases. Although this kind of trajectory can be more in line with physical reality, we find it is not conducive to generating a good mesh. We directly introduce topological priors from a geometric perspective. Overall,  Our topological prior loss consists of two parts:\begin{equation}
    \mathit{L}_{topo} = \lambda_{norm}\mathit{L}_{norm} + \lambda_{flat}\mathit{L}_{flat}
\end{equation}

% 尽管通过上述的物理约束，已经可以实现高斯对人脸相应区域的长距离跟踪。但如果完全严格地让顶点遵从物理约束，会导致个别表情出现顶点的聚集现象。虽然符合物理实际，但是不利于生成良好的网格。{举例说明}。因此顶点的优化还需要考虑拓扑先验。
Firstly, in order to prevent vertex clustering during the optimizing vertex coordinates, we constrain each edge to keep a similar proportion among all connected edges of each vertex:\begin{equation}
\begin{split}
    \mathit{L}_{norm} = \frac{1}{2n_e}\sum_{i\in G}\sum_{j\in ORN_i}|\frac{\Vert\mu_{i,t}-\mu_{j,t}\Vert_2}{\sum_{k\in ORN_i}\Vert\mu_{i,t}-\mu_{k,t}\Vert_2}\\
-\frac{\Vert\mu_{i,0}-\mu_{j,0}\Vert_2}{\sum_{k\in ORN_i}\Vert\mu_{i,0}-\mu_{k,0}\Vert_2}|
\end{split}
\end{equation}

%，我们通过初始帧网格中每个顶点的边长等比例来体现这种先验约束。
% 边长比例损失：{公式和说明}
We find that the above constraints alone cannot guarantee a smooth mesh. We further apply mesh flattening loss\cite{SoftRas} to the geometry to improve mesh quality:\begin{equation}
    \mathit{L}_{flat} = \sum_{\theta_i \in e_i}(cos\theta_i+1)^2
\end{equation}, where $\theta_i$ is the angle between the faces that have the common edge $e_i$. This loss term effectively prevents self-intersection and make the mesh smooth enough.
%我们发现仅仅通过上述约束并不能保证可以从高斯集合提取平滑的网格，我们进一步对几何施加网格平滑损失来提高网格质量。
% 平滑损失：{公式和说明}
% 综上所述：topo loss = edge_norm loss + flat loss
\subsection{Texture Extraction from Gaussians}
\label{sec:Tex Opt}
% 纹理提取与映射：
On the basis of knowing the geometry of each frame, we can naturally learn the color of each Gaussian by Eq. \ref{loss:image}, and then map the learned color to UV space based on the mapping of 3D coordinates to UV coordinates predefined in the topology, generating a Texture map. With the powerful representation ability of Gaussian and the fully optimized Gaussian Rasterizer, we can learn Gaussian colors on 4K multi view images and efficiently generate native 8K textures.
% 在获取了可靠的几何的基础上，我们可以自然而然地通过image损失学习到每个高斯的可靠颜色，进而根据拓扑中三维坐标到UV坐标的映射来将高斯顶点颜色映射到UV空间，生成Texture贴图。借助高斯的强大表征能力和充分优化的高斯Rasterizer，我们可以在4K multiview图像上学习高斯颜色，并高效生成原生8K Texture。

\todo{lift benifit and why}\textbf{UV Space Gaussian Densification.}
Compared to representing geometry, representing pore-level details requires more Gaussians. 3DGS adopts an adaptive densification and pruning process, allowing the density of Gaussians to adaptively change with the complexity of the underlying scene. However, due to the need to maintain topological relationships to achieve inverse texture mapping, similar densification processes cannot be used here. Therefore, we propose a novel densification method, which allows us to insert more Gaussians to Gaussian Mesh. Compared to arbitrarily adding and pruning Gaussians in world space, we choose to insert more Gaussian vertices inside each mesh grid. In this way, we can obtain the UV coordinates corresponding to these new vertices through bilinear interpolation, while connecting edges between these points to maintain topological relationships. Notably, this process is actually equivalent to inserting more sampling points in UV space.

Specifically, we firstly clone the original Gaussian set $G_i$ and only inherit their position/rgb as initialization. It's worth noting that the densified Gaussian set $G_i^{\prime}$ is independent with $G_i$ during optimization. Then for each quadrilateral \textit{Gaussian Grid} in $G_i^{\prime}$, we sequentially insert totally $N \times N-4$ Gaussians ($N-2$ on each edge and $(N-2) \times (N-2)$ inside the grid). The newly generated Gaussian's position/UV/rgb are obtained by bilinear interpolation sampling the corresponding attributes of the original four Gaussians. Each newly generated Gaussian links four edges with its adjacent Gaussians in four directions.

After building the densified Gaussian set $G_i^{\prime}$, We learn their colors and rotations at every frame by Eq. \ref{loss:image}. Due to the fact that in the texture optimization stage, we do not need to focus on rendering quality, but only need to make each Gaussian learn accurate colors and avoid blending, we fix the opacity of each Gaussian to 1, and the scale to the minimum distance between its one-ring neighbours.
%相比于表示几何，表示颜色需要更多的高斯顶点。3DGS采用了自适应的稠密化和删减过程，使高斯顶点的密度随着场景的复杂度自适应地进行变化。然而由于我们需要保持拓扑关系以实现三维坐标到UV坐标的映射，因此无法使用类似的自适应优化过程。相比于在三维空间任意添加和删除高斯顶点，我们选择在每个面片内部插入更多高斯顶点。采用这种方式，我们可以通过双线性插值获取这些新顶点对应的UV坐标，同时在这些点之间连接边来维持拓扑关系。这个过程实际上也相当于在UV空间中进行顶点稠密化。稠密化后的点集可以容易地映射到UV空间。
% UV空间顶点稠密化：具体来说，对于一个四边形面片，我们在各边和中间共有序插入N*N-4个高斯点，position/UV/rgb都在每一帧通过双线性插值采样四角上的顶点属性得到。每个点与其相邻点建立连接关系。对于稠密化后的高斯点集，我们在每一帧都学习其颜色。由于在纹理优化阶段，我们不需要关注渲染质量，而只需要让每个高斯点学习到精确的颜色并避免混合，因此我们设置每个高斯点的opacity为1，scale为其one-ring neighbor间距离的最小值并始终固定不变。

After texture optimization, we can obtain the correspondence between dense world space face colors and UV space colors. we can easily use traditional renderer to render world space colors to UV space and generate texture maps.\todo{formulation}
% 纹理逆映射：优化完纹理颜色后，我们可以得到稠密的三维空间坐标和UV坐标之间的对应关系，以及每个位置精确的纹理颜色。由于我们同时维护了顶点连接关系，可以很容易地使用传统三角面片光栅化渲染方式生成纹理贴图。具体来说：{公式和说明}

==> sections/method_v2.tex <==
\section{Methods}
% \indent{\it Overview.} 
Our method aims to propose a framework to achieve dynamic head meshes and temporal stable textures reconstruction from calibrated multi-view videos. Specifically, given sets of multi-view image sequences $\{ \mathcal{I}^j_i \in \mathbb{R}^{h \times w \times 3} | 1 \leq i \leq F\}_{j=1}^K$ with $F$ frames from $K$ views and known camera calibrations, our method extracts head meshes $\{S_i:=(V^i, T)|V^i\in\mathbb{R}^{n_v\times3}, T\in\mathbb{R}^{n_f\times3} \}_{i=1}^F$ with predefined fixed topology $T$ that has $n_v$ vertices and $n_f$ faces together with 8K texture maps $\{M_i\in\mathbb{R}^{8196\times8196\times3} \}_{i=1}^F$.

To begin with, we give a brief review of 3DGS ~\cite{3DGS} (Sec. \ref{sec:Preliminary}). As is illustrated in figure\todo{Image}, our method first build a \textit{Gaussian Mesh} by initializing a topology integrated Gaussian set based on the geometry and color priors from the first frame (Sec. \ref{sec:Gaussian Mesh}). Then, for each subsequent frame, we alternatively perform geometry optimization by regularizing vertex motion through topology and physics aware loss items and learn dense texture colors by UV space Gaussian densification(Sec. \ref{sec:GTO}). Finally, we extract geometry from a offset \textit{Gaussian Mesh} and render ultra high resolution texture map with pore-level details (Sec. \ref{sec:GTE}).
% Overview：我们的方法基于4DGS优化，输入是一组多视角视频及其相机参数，同时还有通过MVS+Registration方法生成的第一帧人脸几何和贴图。我们用第一帧的贴图和几何初始化高斯点集来构建Gaussian Mesh，为后续的优化过程提供了充分的拓扑、形状和颜色先验。通过物理和拓扑约束，我们优化并跟踪每个高斯点在每一帧的三维位置，从而提取出动态几何。在每一帧我们进行几何和纹理的交替优化，通过UV空间顶点稠密化，我们可以学习精确的顶点颜色并生成原生8K纹理。接下来我们首先介绍GS的前置知识，再给出第一帧初始化并优化Gaussian Mesh的方法。之后我们将详细介绍后续每一帧对几何和纹理的交替优化方法。
\subsection{Preliminary}
\label{sec:Preliminary}
3D Gaussian Splatting (3DGS)~\cite{3DGS} is proposed as a competitive solution to represent and render static scenes. Different from other implicit representation methods, 3DGS explicitly maintains a set of Gaussians to model a scene. By virtue of the explicit intrinsics of Gaussians and the absence of dense MLP execution when sampling from scene representation, 3DGS can render scenes effciently while maintaining high fidelity. Each ellipsoidal Gaussian is described by a covariance matrix $\Sigma$ and its mean position $\mu$:\begin{equation}G(x)=e^{-\frac{1}{2} (x)^T\Sigma ^{-1}(x)}.\end{equation} In order to ensure positive definiteness of the covariance matrix to guarantee its physical meaning during the gradient descent optimization process, $\Sigma$ is further decomposed into rotation matrix $R$ and scaling matrix $S$:\begin{equation}\Sigma=RSS^TR^T,\end{equation} where the rotation matrix is parameterized using a quaternion $q$ for the sake of optimization convenience. In addition to these attributes, each Gaussian also features a learnable color component $c$ and an opacity component $\sigma$ used for rendering.

For rendering, all 3D Gaussians are projected to 2D image plane\cite{zwicker2001ewa}:\begin{equation}\Sigma^\prime=JW\Sigma W^TJ^T,\end{equation} where $W$ is the viewing transformation matrix and $J$ is the Jacobian of the affine approximation of the projective
transformation. Finally, the color $C$ of a pixel is acquired by sampling and blending all Gaussians that overlapping the pixel 
in depth order: \begin{equation}C=\sum_{i=1}c_i\alpha_i\prod_{j=1}^{i-1}(1-\alpha_i),\end{equation} where the blending weight $\alpha_i$
is given by evaluating a 2D Gaussian with its covariance multiplied with its opacity.

However, 3DGS is designed for rendering, not for 3D reconstruction. There is no topological relationship between Gaussians, and unconstrained optimization of their attributes can only produce meaningless geometry, making it impossible to directly extract topologically good meshes.
% Preliminary：GS能从带有位姿的多视角图进行快速高分辨率渲染，通过在第一帧优化高斯的属性，并在后续帧约束这些属性，可以通过多视角图像的变化驱动这些高斯点；{Gaussian Splatting的符号、表示、投影、渲染方程；}
% GS的优势
% GS通过分布在空间中的Gaussian混合颜色实现渲染，然而高斯点之间没有拓扑关系，不加约束地优化三维坐标会导致没有意义的几何形状，无法直接提取拓扑好的mesh和texture；

\subsection{Gaussian Mesh: Topology Integrated Gaussians Initialization}
\label{sec:Gaussian Mesh}
Our goal is to directly extract geometry with consistent topology from Gaussians and its main challenge is the absence of topological constrains in the gradient descent optimization process. The insight behind our method is that Gaussians can render images that reflect the head shape while maintaining topological relationships, so that we can drive Gaussians with topology by multi-view videos. We achieve this by propose \textit{Gaussian Mesh}, novelly integrating topological priors to the initialization and subsequent frame by frame optimization process of vanilla Gaussians. 
% To build a Gaussian Mesh consist of two steps: \textbf{Facial Shape Binding} and \textbf{Facial Color Occupying}.

\input{Tables/Attributes} 
% \indent{\it Facial Shape Binding.} 
Firstly, we bind Gaussians to the underlying head surface. Different from 3DGS using SFM to generate sparse point clouds for Gaussian initialization, our method begins from a head mesh and texture of the first frame, which is acquired by an off the shelf automatic MVS and registration method. Since the mesh and texture of the first frame provide reliable geometry information, together with the predefined topology, we initialize Gaussians $G_1=\{G_{1,i}\}_{i=1}^{n_v}$ with the same number of vertices as the mesh, and set the mean position of Gaussians to the vertex 3D world space coordinates in topological order. In order to align Gaussians with the surface as close as possible, we set the the orientation of each Gaussian to be the same as the normal direction of the mesh vertices.

% At the same time, in order to avoid color blending between multiple Gaussians as much as possible, and to form a one-to-one correspondence between the facial region and the Gaussians, we initialize the scales $s$ as half of the minimum distance between each vertex and its one-ring neighbors ($ORN$), and set opacity $\sigma$ to 1. All in all, the proposed Gaussian Mesh is composed of a set of constrained optimized Gaussians as shown in Tab. \ref{tbl:attributes}.
% Topology Integrated Gaussians initialization：与普通的3DGS使用SFM产生的稀疏点云初始化高斯点集不同，我们首先用传统MVS+Fitting的方式重建出第一帧的mesh和texture作为拓扑和颜色先验，再将Gaussian分布绑定到第一帧的人脸网格。由于希望能够从高斯点的位置直接提取出几何，我们创建与网格顶点数目相同的高斯点，将高斯的mean position按照拓扑顺序设置为网格顶点坐标；同时为了尽可能避免多个高斯间的颜色混合，使面部区域与高斯点集尽可能构成一一对应，我们将scale初始化为每个顶点与其one-ring neighbour距离的最小值，并设置每个高斯的opacity为1；

By attaching Gaussians to head mesh vertices, we only initialize the shape related attributes (i.e. mean position and rotation). We then need to optimize their color related attributes (i.e. scale, opacity and color).
% through \textbf{Facial Color Occupying}.
% \todo{}Notably, GaussianAvatar~\cite{GaussianAvatar} also utilizes face priors by rigging Gaussians to explicit head mesh, and drive it by FLAME\cite{FLAME} parameters. However \cite{GaussianAvatar} rigs multiple Gaussians to mesh faces while we bind a single Gaussian to each vertex and build a a one-to-one mapping between Gaussians and vertices according to the topology. 
% \indent{\it Facial Color Occupying.}The logic behind facial color occupying is to make each Gaussian represent a small region of the face independently, so that the movement of the face in the videos can reflect the movement of the corresponding Gaussians. To achieve this, 
We initialize the scales $s_0$ as half of the minimum distance between each Gaussian and its one-ring neighbours ($ORN$), and set opacity $\sigma$ to 1, avoiding color blending between multiple Gaussians as much as possible. Since the texture provide true color of the head, we set each Gaussian's color by sampling from the texture map according to the UV coordinate of each vertex. Finally, we optimize Gaussian's scale by rendering the images of the first frame. We adopt the same image loss as 3DGS:\begin{equation}\label{loss:image}\mathit{L}_{image} = (1-\lambda ) \mathit{L}_{1} + \lambda\mathit{L}_{D-SSIM},\end{equation} where $\lambda$ is always set to 0.2 and all other attributes are fixed except for rotation and scale during this process.

A Gaussian is like an ellipsoid but a point without volume, and its mean position does not represent the true position of the surface it renders. If we want to extract geometry from Gaussians, we need to hypothesize that the Gaussians are like flat ellipses and aligned with the underlying head surface closely. This actually requires constraining one direction of Gaussian's scale close to 0 and penalize Gaussians have excessive size:\begin{equation}\mathit{L}_{scale} = \sum_{i\in G}(\Vert s_i \Vert_{-\infty} + max(0, s_i -1.5s_{i,0})),\end{equation} where Gaussian with scale exceeding 1.5 times the initial value $s_0$ will be penalized.

Overall, the final loss for facial color occupying can be formulated as:\begin{equation}\mathit{L}_{init} = \mathit{L}_{image} + \lambda_{scale} \mathit{L}_{scale}.\end{equation}
% 初始帧优化目标：由于已知第一帧的可靠几何和颜色先验，因此我们在第一帧只优化高斯的scale、rotation。初始帧优化阶段使用和3DGS相同的image损失（L1loss + ssim）:{公式和说明}
%scale损失：{公式和说明}
%接下来我们具体介绍后续帧的几何优化。
\subsection{Alternating Geometry and Texture Optimization}
\label{sec:GTO}
Since we have built a initial Gaussian Mesh $G_1$ in Sec. \ref{sec:Gaussian Mesh}, we then acquire Gaussian Mesh $G_i$ at frame $i$ by optimizing $G_{i-1}$ at the previous frame. Specifically, we perform \textit{Alternating Geometry and Texture Optimization} frame by frame, where we obtain geometry by driving Gaussians under the regularization of topology and physics and learn dense texture colors on the basis of current frame's geometry.

\subsubsection{Geometry Optimization}\label{sec:geo opt} To maintain the topology relationships within Gaussians while keeping long-term tracks and rendering quality, we extend 3DGS by introducing physical and topological priors to the opimization objectives. Specifically, we propose physical loss item $\mathit{L}_{phy}$ that constrain local rigidity and topological loss $\mathit{L}_{topo}$ that improve the mesh quality.
Overall, the loss items for geometry optimization is constructed by three parts: \begin{equation}
    \mathit{L}_{geo} = \mathit{L}_{image} + \mathit{L}_{phy} + \mathit{L}_{topo},
\end{equation} where the image loss is illustrated as Eq. \ref{loss:image}.
%通过在第一帧用可靠先验初始化高斯的rgb/position，同时设置opacity为1，可以使得每个3D高斯表示人脸相应位置的物理成分；通过在后续帧限制高斯scale，同时放开rotation和position、可以建模人脸相应物理成分的运动。
% 值得注意的是，相同的面部区域会随着表情的不同产生不同的阴影颜色，因此我们放开rgb的学习，有助于建模由于人脸动态运动导致的阴影和褶皱。第一帧的面部颜色先验无法给予这部分信息，但是对识别人脸几何十分重要。

\indent{a) Physical Prior Loss.} The correspondence between Gaussians and facial regions achieved by color occupying \ref{sec:Gaussian Mesh} is weak. For example, for regions such as forehead and cheek, where the color is similar and the geometry is relatively flat, a Gaussian can freely represent similar physical areas, leading to incorrect tracking relationships. This means that in addition to indirectly optimizing Gaussian positions through differentiable rendering, physical priors are needed to regularize the motion of Gaussians directly. Following the practice of \cite{DynamicGaussian} but with some modifications, our physical prior loss consists of three parts:\begin{equation}
    \mathit{L}_{phy} = \lambda_{rigid}\mathit{L}_{rigid} + \lambda_{rot}\mathit{L}_{rot} + \lambda_{iso}\mathit{L}_{iso},
\end{equation} where $\mathit{L}_{rigid}$ and $\mathit{L}_{rot}$ are used to regularize short-term local-rigidity and rotation
similarity of Gaussians, respectively, and $\mathit{L}_{iso}$ is a long-term local-isometry loss. We refer readers to \cite{DynamicGaussian} for more details about the original design of these loss terms.

% 只通过冻结高斯的部分属性来实现高斯和人脸对应位置的绑定是不可靠的，例如对于额头、脸颊等区域，颜色相同且几何较为平整，一个高斯可以自由地表征相似的物理区域，导致错误的跟踪关系。
The physical loss between Gaussians should under the priors of topology for we don't want a Gaussian to affect all nearby Gaussians blindly, e.g. a Gaussian on the upper lip and a Gaussian on the lower lip but closest to it. Therefore, unlike \cite{DynamicGaussian}, we only impose such loss between one-ring neighbours:\begin{equation}
    \mathit{L}_{rigid}(i, j)=w_{i, j}\Vert(\mu_{j,t-1}-\mu_{i,t-1})-R_{i,t-1}R_{i,t}^{-1}(\mu_{j,t}-\mu_{i,t})\Vert_2
\end{equation}
\begin{equation}
    \mathit{L}_{rigid}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} \mathit{L}_{rigid}(i,j)
\end{equation}, where $n_e$ is the number of edges and $ORN_i$ means the one-ring neighbours of $G_i$. The loss weighing factor takes into account the edge length of the Gaussian Mesh at the first frame:\begin{equation}
    w_{i, j}=exp(-\lambda_w\Vert\mu_{j, 0}-\mu_{i,0}\Vert_2^2).
\end{equation}

% 刚体距离损失：{公式和说明}
We also regularize Gaussian's rotation in a similar manner:\begin{equation}
     \mathit{L}_{rot}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} w_{i,j}\Vert\hat q_{j, t}\hat q_{j, t-1}^{-1}-\hat q_{i, t}\hat q_{i, t-1}^{-1}\Vert_2,
\end{equation} where $\hat q$ is the normalized quaternion.

% 刚体旋转损失：{公式和说明}
In addition to the loss terms mentioned above that are only calculated between adjacent frames, we find that long-term physical loss is important for maintaining long-distance topological consistency after doing expressions, for it strongly introduces the topology priors about the edge length:\begin{equation}
    \mathit{L}_{iso}=\frac{1}{2n_e} \sum_{i\in G}\sum_{j\in ORN_i} w_{i,j}|\Vert\mu_{j,0}-\mu_{i,0}\Vert_2-\Vert\mu_{j,t}-\mu_{i,t}\Vert_2|.
\end{equation}

% 刚体长距离损失：{公式和说明}
\indent{b) Topology Prior Loss.} By means of the physical constraints mentioned above, our method is able to achieve long-term tracking of the corresponding face regions. But if vertices are strictly constrained by physical constraints, it can lead to bad wiring and unsmooth surfaces. Therefore, we introduce topological priors to regularize vertex motion. Specifically, we consider both the distance constraint between each vertex and its one-ring neighbours, as well as the angle constraint between each face and its adjacent faces.

% 尽管通过上述的物理约束，已经可以实现高斯对人脸相应区域的长距离跟踪。但如果完全严格地让顶点遵从物理约束，会导致个别表情出现顶点的聚集现象。虽然符合物理实际，但是不利于生成良好的网格。{举例说明}。因此顶点的优化还需要考虑拓扑先验。

% Firstly, we constrain each edge to keep a similar proportion among all connected edges of each vertex:\begin{equation}
% \begin{split}
%     \mathit{L}_{norm} = \frac{1}{2n_e}\sum_{i\in G}\sum_{j\in ORN_i}|\frac{\Vert\mu_{i,t}-\mu_{j,t}\Vert_2}{\sum_{k\in ORN_i}\Vert\mu_{i,t}-\mu_{k,t}\Vert_2}\\
% -\frac{\Vert\mu_{i,0}-\mu_{j,0}\Vert_2}{\sum_{k\in ORN_i}\Vert\mu_{i,0}-\mu_{k,0}\Vert_2}|.
% \end{split}
% \end{equation}

% %，我们通过初始帧网格中每个顶点的边长等比例来体现这种先验约束。
% % 边长比例损失：{公式和说明}
% We find that the above constraints alone cannot guarantee a smooth mesh. We further apply mesh flattening loss\cite{SoftRas} to the geometry to improve mesh quality:\begin{equation}
%     \mathit{L}_{flat} = \sum_{\theta_i \in e_i}(cos\theta_i+1)^2,
% \end{equation} where $\theta_i$ is the angle between the faces that have the common edge $e_i$. This loss term effectively prevents self-intersection and make the mesh smooth enough.

To prevent the vertices from moving freely, we calculate L2 loss between the position of each vertex and the average position of its neighbours:\begin{equation}
    \mathit{L}_{pos}=\frac{1}{n_v}\sum_{i\in G}(\mu_i-\frac{ {\textstyle \sum_{j\in ORN_i}\mu_j} }{|ORN_i|} )^2
\end{equation}

We further apply mesh flattening loss to encourage the angle between adjacent faces to remain constant with the first frame during the optimization process:\begin{equation}
    \mathit{L}_{flat} = \sum_{\theta_i \in e_i}(1-cos(\theta_{i,t}-\theta_{i,0})),
\end{equation} where $\theta_{i,t}$ is the angle between the faces that have the common edge $e_i$ at frame t. This loss term effectively prevents self-intersection and make the mesh smooth enough.

Overall,  our topological prior loss consists of two parts:\begin{equation}
    \mathit{L}_{topo} = \lambda_{pos}\mathit{L}_{pos} + \lambda_{flat}\mathit{L}_{flat}.
\end{equation}

\indent{c) Learning Strategy.} The learning strategy for each attribute are illustrated in Tab. \ref{tbl:attributes}. By freezing the scale in subsequent frames while releasing rotation and position, the motion of the corresponding physical components of the face can be modeled. It is worth noting that the same facial region will produce different colors when doing different expressions, e.g. ambient occlusion around wrinkles. Therefore, by allow Gaussian's color change during optimization, we can to some extent model shadows caused by self occlusion. The facial color prior in the first frame cannot reflect this phenomenon, but it is crucial for recognizing facial geometry.
%我们发现仅仅通过上述约束并不能保证可以从高斯集合提取平滑的网格，我们进一步对几何施加网格平滑损失来提高网格质量。
% 平滑损失：{公式和说明}
% 综上所述：topo loss = edge_norm loss + flat loss
\input{Figures/dense}
\subsubsection{Texture Optimization}\label{sec:tex opt} After geometry optimization, we have obtained the geometry of each frame, and also the color of each Gaussian that can represent the head coarsely. Compared to representing geometry, representing pore-level details and generating 8K texture map requires more Gaussians learning on 4K images. 3DGS adopts an adaptive densification and pruning process, allowing the density of Gaussians to adaptively change with the complexity of the underlying scene. However, due to the need to maintain topological relationships to achieve inverse texture mapping, similar densification processes cannot be used here. We thus propose a novel densification method i.e. \textbf{UV Space Densification}, which allows us to insert more Gaussians to Gaussian Mesh without destroying the topology.

\indent{a) UV Space Densification.} We build a dense Gaussian Mesh $G^{\prime}$ by inserting Gaussians to the original Gaussian Mesh $G$. It's worth noting that $G^{\prime}$ is independent with $G$ and we only optimize $G^{\prime}$ during texture optimization. Specifically, we firstly clone $G$ and only inherit their position/rgb as initialization. Then for each quadrilateral mesh grid in $G^{\prime}$, we sequentially insert totally $N \times N-4$ Gaussians ($N-2$ on each edge and $(N-2) \times (N-2)$ inside the grid). \todo{Image}The newly generated Gaussian's position, UV coordinates, and color are obtained by bilinear interpolation sampling the corresponding attributes of the four Gaussians (e.g. $G_{0, 0}^{\prime}$, $G_{0, N-1}^{\prime}$, $G_{N-1, 0}^{\prime}$ and $G_{N, N}^{\prime}$) at the grid vertices:\begin{equation}\label{eq:sampling}\begin{split}
A_{i, j} = \frac{1}{(N-1)\times (N-1)}
\begin{bmatrix}
 N-1-i & i
\end{bmatrix}\\
\begin{bmatrix}
 A_{0,0} & A_{0,N-1}\\
 A_{N-1,0} & A_{N-1,N-1}
\end{bmatrix}
\begin{bmatrix}
 N-1-j\\
 j
\end{bmatrix},
\end{split}
\end{equation} where A can be $c$/uv/$\mu$. Most importantly, in addition to interpolating to obtain UV coordinates, it is also easy to establish connection relationships between Gaussians. For example, $G_{i, j}$ is connected to $G_{i-1, j}$, $G_{i+1, j}$, $G_{i, j-1}$ and $G_{i, j+1}$. This process is actually equivalent to subdividing the grid and inserting more sampling points in UV space.

\indent{b) Learning Strategy.} For dense Gaussian Mesh $G_i^{\prime}$ at frame $i$, we follow a similar pratice as we do in Sec. \ref{sec:Gaussian Mesh}. Specifically, we sampling each Gaussian's $\mu$ by Eq. \ref{eq:sampling} and set their opacity to 1. The rotation and color are inherited from previous frame, thus the texture optimization process does not require too many iterations. Since we only need to learn the exact color of the UV space sampling points represented by each Gaussian, we dont't expand Gaussian's scale here and only fix it to be the minimum distance with one-ring neighbours. The training objective is the same as Eq. \ref{loss:image} and we perform optimizing at 4K resolution.

% 纹理提取与映射：
% 在获取了可靠的几何的基础上，我们可以自然而然地通过image损失学习到每个高斯的可靠颜色，进而根据拓扑中三维坐标到UV坐标的映射来将高斯顶点颜色映射到UV空间，生成Texture贴图。借助高斯的强大表征能力和充分优化的高斯Rasterizer，我们可以在4K multiview图像上学习高斯颜色，并高效生成原生8K Texture。

% \todo{lift benifit and why}\textbf{UV Space Gaussian Densification.}
%  Compared to arbitrarily adding and pruning Gaussians in world space, we choose to insert more Gaussian vertices inside each mesh grid. In this way, we can obtain the UV coordinates corresponding to these new vertices through bilinear interpolation, while connecting edges between these points to maintain topological relationships. This process is actually equivalent to inserting more sampling points in UV space.


% After building the densified Gaussian set $G_i^{\prime}$, We learn their colors and rotations at every frame by Eq. \ref{loss:image}. Due to the fact that in the texture optimization stage, we do not need to focus on rendering quality, but only need to make each Gaussian learn accurate colors and avoid blending, we fix the opacity of each Gaussian to 1, and the scale to the minimum distance between its one-ring neighbours.
%相比于表示几何，表示颜色需要更多的高斯顶点。3DGS采用了自适应的稠密化和删减过程，使高斯顶点的密度随着场景的复杂度自适应地进行变化。然而由于我们需要保持拓扑关系以实现三维坐标到UV坐标的映射，因此无法使用类似的自适应优化过程。相比于在三维空间任意添加和删除高斯顶点，我们选择在每个面片内部插入更多高斯顶点。采用这种方式，我们可以通过双线性插值获取这些新顶点对应的UV坐标，同时在这些点之间连接边来维持拓扑关系。这个过程实际上也相当于在UV空间中进行顶点稠密化。稠密化后的点集可以容易地映射到UV空间。
% UV空间顶点稠密化：具体来说，对于一个四边形面片，我们在各边和中间共有序插入N*N-4个高斯点，position/UV/rgb都在每一帧通过双线性插值采样四角上的顶点属性得到。每个点与其相邻点建立连接关系。对于稠密化后的高斯点集，我们在每一帧都学习其颜色。由于在纹理优化阶段，我们不需要关注渲染质量，而只需要让每个高斯点学习到精确的颜色并避免混合，因此我们设置每个高斯点的opacity为1，scale为其one-ring neighbor间距离的最小值并始终固定不变。

% After texture optimization, we can obtain the correspondence between dense world space face colors and UV space colors. we can easily use traditional renderer to render world space colors to UV space and generate texture maps.\todo{formulation}
% 纹理逆映射：优化完纹理颜色后，我们可以得到稠密的三维空间坐标和UV坐标之间的对应关系，以及每个位置精确的纹理颜色。由于我们同时维护了顶点连接关系，可以很容易地使用传统三角面片光栅化渲染方式生成纹理贴图。具体来说：{公式和说明}
\subsection{Extracting Geometry and Texture from Gaussians}
\label{sec:GTE}
Once alternating geometry and texture optimization is done, we can finally extract geometry from $G_i$ and extract 8K texture map from $G_i^{\prime}$.

\subsubsection{Geometry Extraction} Since a Gaussian is equivalent to an ellipsoid in 3D space, the surface rendered by Gaussian and the geometric surface formed by Gaussian mean positions are not the same, and the latter tends to be enveloped by the former. In order to make the surface extracted from Gaussians closer to the real surface, we offset each Gaussian along vertex normal direction to get the final mesh vertex: \begin{equation}
        n^{\prime} = R^{-1}n,
    \end{equation} 
    \begin{equation}
        \mu{\prime} = \mu + \sqrt{\frac{1}{\frac{n_x^{\prime 2}}{s_x^2}+\frac{n_y^{\prime 2}}{s_y^2}+\frac{n_z^{\prime 2}}{s_z^2}} }n,
    \end{equation}
where $n$ is the corresponding vertex normal of each Gaussian and we omit vertex numbering. Specifically, as is shown in \todo{Image}, we offset each Gaussian's mean position by its distance from the surface of the ellipsoid in the vertex normal direction. Finally, we compensate for errors caused by Gaussian scale and acquire the head mesh.

\subsubsection{Texture Extraction} To generate 8K texture map from dense Gaussian Mesh $G^{\prime}$ is to inverse map their colors according to their uv coordinates and interpolate each pixel's color. Since we also maintain the topology between Gaussians in Sec. \ref{sec:tex opt}, we can triangulate the Gaussian Mesh and then directly render the texture map using traditional rasterization based rendering. Denoting the Gaussian indices of the triangle visible in pixel $(x, y)$ by $i_{0,1,2}$, and the
barycentrics by $w_{0,1,2}$. The pixel color at $(x, y)$ can be computed by:\begin{equation}
    C_{x,y}=w_0c_{i_0} + w_1c_{i_1} + (1-w_0-w_1)c_{i_2}.
\end{equation}

By extracting geometry and texture map frame by frame, our framework can generate dynamic high-fidelity head mesh together with temporal consistant ultra-high resolution texture map with pore-level details.



